Alternating Local Enumeration (TnALE): Solving Tensor Network Structure Search with Fewer Evaluations

Tensor network (TN) is a powerful framework in machine learning, but selecting a good TN model, known as TN structure search (TN-SS), is a challenging and computationally intensive task. The recent approach TNLS~\cite{li2022permutation} showed promising results for this task, however, its computational efficiency is still unaffordable, requiring too many evaluations of the objective function. We propose TnALE, a new algorithm that updates each structure-related variable alternately by local enumeration, \emph{greatly} reducing the number of evaluations compared to TNLS. We theoretically investigate the descent steps for TNLS and TnALE, proving that both algorithms can achieve linear convergence up to a constant if a sufficient reduction of the objective is \emph{reached} in each neighborhood. We also compare the evaluation efficiency of TNLS and TnALE, revealing that $\Omega(2^N)$ evaluations are typically required in TNLS for \emph{reaching} the objective reduction in the neighborhood, while ideally $O(N^2R)$ evaluations are sufficient in TnALE, where $N$ denotes the tensor order and $R$ reflects the \emph{``low-rankness''} of the neighborhood. Experimental results verify that TnALE can find practically good TN-ranks and permutations with vastly fewer evaluations than the state-of-the-art algorithms.

==> 30_ALGORITHM/AlgoALS.tex <==
\begin{algorithm}[tb]
  \caption{Alternating local sampling, \emph{the core process}}
  \label{alg:ALS}
\begin{algorithmic}
  \STATE {\bfseries Input:}
  A neighborhood center at $(G_0,\mathbf{r}_0)$, where $\mathbf{r}_0\in\mathbb{Z}^{+,\vert{}E\vert}$; maximum number of iterations: $\#Iter$;
  \STATE {\bfseries Initialize:}
  Set $\mathbf{r}=r_0$; $G=G_0$.
  \WHILE{$l\leq{}\#Iter$}
  \FOR{$k=1,2,\ldots,\vert{}E\vert$} 
  \STATE 1. Sampling TN structures by fixing $(G,\mathbf{r})$ but enumerating $\mathbf{r}(k)$ in the neighborhood;
  \STATE 2. Sample evaluation with the objective of~\eqref{eq:basicModel};
  \STATE 3. Update $\mathbf{r}(k)$ using the sample of the smallest objective;
  \ENDFOR
  \STATE 4. Update $G$ similarly as the steps 1-3;
  \FOR{$k=\vert{}E\vert,\vert{}E\vert-1,\ldots,2$}
  \STATE Repeat the steps 1-3;
  \ENDFOR
  \STATE $l=l+1$;
  \ENDWHILE
  \STATE {\bfseries Output:} $(G,r)$ with smallest value of the objective function in all samples.
\end{algorithmic}
\end{algorithm}

==> 50_EXPERIMENTS/TNPSlong.tex <==
\begin{table}[tb]
	\centering
	\caption{
	Evaluation cost in the experiment for the rank and permutation identification, where the symbol ``-'' in the table means the failure in identification.
% 	In the table, \emph{Eff.} denotes the parameter efficiency defined in~\cite{li2020evolutionary},
% 	$\#Eva.$ denotes the number of evaluations, and the ``-'' denotes that the methods fail to satisfy the condition $RSE\leq{}10^{-4}$.
% 	Experimental results of searching structures on synthetic data in various TN format.
% 	In the table the meaning of the values (in different types of brackets) is the same as Table~\ref{tab:TR}.
% 	In the table, \emph{Eff.} denotes the parameter ratio between the structures by different methods and the ground-truths; \emph{RSE} in round brackets indicates the relative square error (ignored if smaller than $10^{-4}$.) and \emph{Gen.} in angle brackets indicates the generation of the reported individual of our methods.
% 	For rows, ``ranks'' means that we fix the permutation as identity yet only searching the ranks, while ``ranks+matching'' means that both the optimal ranks and permutation are taken into account.
	}
 \label{Tab:TNPS}
	\vskip 0.15in
	\begin{threeparttable}\footnotesize
		\setlength{\tabcolsep}{1.5mm}{   	
			\begin{tabular}{llcccc}
				\toprule
	\multirow{2}[0]{*}{\textbf{Topology}}&\multirow{2}[0]{*}{\textbf{Methods}}&\multicolumn{4}{c}{\textbf{Data} -- \emph{\#Eva.~$\downarrow$} }\\
				\cmidrule{3-6}&
				& \textbf{A} & \textbf{B} & \textbf{C}  & \textbf{D} \\
				\midrule
				
				\multirow{3}[0]{*}{\textbf{TR}~(order-4)}
				% &\textit{ranks}&0.40~$\langle{}$005$\rangle{}$~[600]&0.41~(0.02)~$\langle{}$008$\rangle{}$~[960]&0.40~(9e-3)~$\langle{}$006$\rangle{}$~[720]&0.65~(0.04)~$\langle{}$005$\rangle{}$~[600] \\
				% \vspace{0.1cm}
				&TNGA+&450&450&450&300
				\\
				% \vspace{0.1cm}
				&TNLS&240&300&60&300
				\\
				&Ours&\textbf{93}&\textbf{155}&\textbf{31}&\textbf{124}
				
				% \\\vspace{0.1cm}	&\textcolor{red}{\textit{Greedy}}&\textcolor{red}{1.29~(T-Tree)}&\textcolor{red}{1.03}&\textcolor{red}{0.79}&\textcolor{red}{1.27} 
				\\
				% \midrule
				\cmidrule{2-6}
				
			
				\multirow{3}[0]{*}{\textbf{TR}~(order-6)}
				% &\textit{ranks}&0.72~(0.01)~$\langle{}$012$\rangle{}$~[1440]&0.95~$\langle{}$011$\rangle{}$~[1320]&1.93~$\langle{}$011$\rangle{}$~[1320]&0.65~(0.04)~$\langle{}$014$\rangle{}$~[1680] \\
				&TNGA+&1500&1350&1650&1650
				\\
				% \vspace{0.1cm}
				&TNLS&660&600&660&600
				\\
				% \vspace{0.1cm}
				&Ours&\textbf{156}&\textbf{321}&\textbf{156}&\textbf{156}
				\\
                \cmidrule{2-6}

                \multirow{3}[0]{*}{\textbf{TR}~(order-8)}
				% &\textit{ranks}&0.72~(0.01)~$\langle{}$012$\rangle{}$~[1440]&0.95~$\langle{}$011$\rangle{}$~[1320]&1.93~$\langle{}$011$\rangle{}$~[1320]&0.65~(0.04)~$\langle{}$014$\rangle{}$~[1680] \\
				&TNGA+&2850&2250&3900&1950
				\\
				% \vspace{0.1cm}
				&TNLS&1020&960&1320&780
				\\
				% \vspace{0.1cm}
				&Ours&\textbf{231}&\textbf{308}&\textbf{308}&\textbf{231}
				\\
                \cmidrule{2-6}

                \multirow{3}[0]{*}{\textbf{PEPS}}
				% &\textit{ranks}&0.72~(0.01)~$\langle{}$012$\rangle{}$~[1440]&0.95~$\langle{}$011$\rangle{}$~[1320]&1.93~$\langle{}$011$\rangle{}$~[1320]&0.65~(0.04)~$\langle{}$014$\rangle{}$~[1680] \\
				&TNGA+&1560&-&840&1080
				\\
				% \vspace{0.1cm}
				&TNLS&781&781&421&661
				\\
				% \vspace{0.1cm}
				&Ours&\textbf{407}&\textbf{465}&\textbf{233}&\textbf{175}
				\\
                \cmidrule{2-6}

                \multirow{3}[0]{*}{\textbf{HT}}
				% &\textit{ranks}&0.72~(0.01)~$\langle{}$012$\rangle{}$~[1440]&0.95~$\langle{}$011$\rangle{}$~[1320]&1.93~$\langle{}$011$\rangle{}$~[1320]&0.65~(0.04)~$\langle{}$014$\rangle{}$~[1680] \\
				&TNGA+&960&1320&840&1080
				\\
				% \vspace{0.1cm}
				&TNLS&841&841&781&721
				\\
				% \vspace{0.1cm}
				&Ours&\textbf{211}&\textbf{281}&\textbf{211}&\textbf{211}
				\\
                \cmidrule{2-6}

                \multirow{3}[0]{*}{\textbf{MERA}}
				% &\textit{ranks}&0.72~(0.01)~$\langle{}$012$\rangle{}$~[1440]&0.95~$\langle{}$011$\rangle{}$~[1320]&1.93~$\langle{}$011$\rangle{}$~[1320]&0.65~(0.04)~$\langle{}$014$\rangle{}$~[1680] \\
				&TNGA+&-&960&2800&3240
				\\
				% \vspace{0.1cm}
				&TNLS&1561&841&1441&721
				\\
				% \vspace{0.1cm}
				&Ours&\textbf{1450}&\textbf{484}&\textbf{323}&\textbf{323}
				\\
                \cmidrule{2-6}

                \multirow{3}[0]{*}{\textbf{TW}}
				% &\textit{ranks}&0.72~(0.01)~$\langle{}$012$\rangle{}$~[1440]&0.95~$\langle{}$011$\rangle{}$~[1320]&1.93~$\langle{}$011$\rangle{}$~[1320]&0.65~(0.04)~$\langle{}$014$\rangle{}$~[1680] \\
				&TNGA+&1920&1440&600&720
				\\
				% \vspace{0.1cm}
				&TNLS&661&601&601&481
				\\
				% \vspace{0.1cm}
				&Ours&\textbf{285}&\textbf{143}&\textbf{285}&\textbf{214}
				\\
                % \cmidrule{2-6}

    
				\bottomrule
				
			\end{tabular}
		}
	\end{threeparttable}
	\vskip -0.1in
\end{table}
